Contrastive Video Question Answering via Video Graph Transformer

We propose to perform video question answering (VideoQA) in a Contrastive manner via a Video Graph Transformer model (CoVGT). CoVGT's uniqueness and superiority are three-fold: 1) It proposes a dynamic graph transformer module which encodes video by explicitly capturing the visual objects, their relations and dynamics, for complex spatio-temporal reasoning. 2) It designs separate video and text transformers for contrastive learning between the video and text to perform QA, instead of multi-modal transformer for answer classification. Fine-grained video-text communication is done by additional cross-modal interaction modules. 3) It is optimized by the joint fully- and self-supervised contrastive objectives between the correct and incorrect answers, as well as the relevant and irrelevant questions respectively. With superior video encoding and QA solution, we show that CoVGT can achieve much better performances than previous arts on video reasoning tasks. Its performances even surpass those models that are pretrained with millions of external data. We further show that CoVGT can also benefit from cross-modal pretraining, yet with orders of magnitude smaller data. The results demonstrate the effectiveness and superiority of CoVGT, and additionally reveal its potential for more data-efficient pretraining. We hope our success can advance VideoQA beyond coarse recognition/description towards fine-grained relation reasoning of video contents. Our code is available at https://github.com/doc-doc/CoVGT.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/experiments_bak.tex <==
% !TEX root = ../main.tex

%--------------------------------------------------------
\section{Experiments}
\label{sec:exp}

\setlength{\tabcolsep}{6pt}
\begin{table*}[t]
    \small
    \centering
    \caption{Accuracy (\%) comparison on NExT-QA \cite{xiao2021next}. F: Frame representation from ResNet or its variants. C: Clip representation from 3D networks like I3D \cite{carreira2017quo,hara2018can} and S3D \cite{xie2018rethinking}, C$^+$: cross-modal pretrained S3D \cite{miech2020end}. R: Region representation from Faster R-CNN with ResNet backbone. BERT: BERT \cite{devlin2018bert} or its variants \cite{sanh2019distilbert}. Acc@C, T, D, denote accuracy for Causal, Temporal and Descriptive questions respectively; the corresponding proportion of data are also given. *:results reproduced by us with official code. The best results and previous SoTA results are highlighted in bold and underline respectively.
    }
    \vspace{-0.5em}
    \scalebox{0.9}{
    \begin{tabular}{l|cc|c|c|ccc|c|ccc|c}
    \hline\hline
    \multirow{3}*{Methods} & \multicolumn{2}{c|}{\multirow{1}*{Pretrain}}& \multirow{3}*{Video} & \multirow{3}*{Text} & \multicolumn{4}{c|}{NExT-QA Val} & \multicolumn{4}{c}{NExT-QA Test} \\ \cline{2-3} \cline{6-13}
    ~ & \multirow{2}*{Dataset} & \multirow{2}*{Size} & ~ & ~ & Acc@C & Acc@T & Acc@D & \multirow{2}*{Acc@All} & Acc@C & Acc@T & Acc@D & \multirow{2}*{Acc@All} \\ 
     ~ & ~ & ~ & ~ & ~ & (48\%) & (29\%) & (23\%) & ~ & (48\%) & (29\%) & (23\%) & ~ \\ 
    \hline
    STVQA \cite{jang2017tgif} & - & - &F, C &BERT & 44.76 & 49.26 & 55.86 & 47.94 & 45.51 & 47.57 & 54.59 & 47.64 \\
    CoMem \cite{gao2018motion} & - & - &F, C &BERT & 45.22 & 49.07 & 55.34 & 48.04 & 45.85 & 50.02 & 54.38 & 48.54 \\
    HCRN \cite{le2020hierarchical} & - & - & F, C &BERT & 45.91 & 49.26 & 53.67 & 48.20 & 47.07 & 49.27 & 54.02 & 48.89 \\
    HME\cite{fan2019heterogeneous}  & - & -  &F, C & BERT & 46.18 & 48.20 & 58.30 & 48.72 & 46.76 & 48.89 & 57.37 & 49.16 \\
    HGA \cite{jiang2020reasoning} & - & - & F, C &BERT & 46.26 & 50.74 & 59.33 & 49.74 & 48.13 & 49.08 & 57.79 & 50.01 \\
    HQGA \cite{xiao2021video} & - & - & R, F, C &BERT &48.48 & 51.24 & 61.65 & 51.42 & \underline{49.04} & \underline{52.28} & 59.43 & \underline{51.75} \\
    P3D-G \cite{cherian2022} &- & - & R, C &BERT & \underline{51.33} & \underline{52.30} & 62.58 & \underline{53.40} & - & -& -& - \\
    VQA-T* \cite{yang2021just} & - & - & C^+ & BERT & 41.66 & 44.11 & 59.97 & 45.30 & 42.05 & 42.75 & 55.87 & 44.54 \\
    VQA-T* \cite{yang2021just} & How2VQA& 69M & C^+ & BERT & 49.60 & 51.49 & \underline{63.19} & 52.32 & 47.89 & 50.02 & \underline{61.87} & 50.83 \\
   
    \hline
    \multirow{2}*{\textbf{VGT (Ours)}} & - & - &R, F &BERT & 52.28 & 55.09 & 64.09 & 55.02 & 51.62 & 51.94 & 63.65 & 53.68 \\
  
     ~ & WebVid & 0.18M &R, F &BERT & \textbf{53.43} & {\bf56.39} & \textbf{69.50} & \textbf{56.89} & \textbf{52.78} & \textbf{54.54} & \textbf{67.26} & \textbf{55.70} \\ \hline
     \multicolumn{5}{c|}{Improvements (\%)} & \textcolor{red}{+2.1} & \textcolor{red}{+4.1} & \textcolor{red}{+6.3} & \textcolor{red}{+3.5} & \textcolor{red}{+3.7} & \textcolor{red}{+2.3} & \textcolor{red}{+5.4} & \textcolor{red}{+4.0} \\ \hline
    \end{tabular}
    }
    \label{tab:resnextqa}
    \vspace{-0.5em}
\end{table*}
%--------------------------------------------------------
\subsection{Datasets and Tasks}
To validate our model's effectiveness, we conduct experiments on 5 VideoQA benchmarks across 11 task that challenge the various aspects of video understanding: 
\begin{enumerate}
    \item NExT-QA \cite{xiao2021next} is a manually annotated dataset that benchmarks a comprehension of the causal and temporal object interaction in space-time. Its videos are sourced from VidOR \cite{shang2019annotating} and cover various daily activities. Each question has 5 options with 1 correct answer and 4 distractor answers.
    \item STAR-QA \cite{wu2021star} benchmarks situated visual reasoning in real-world scenes. It is based on Action Genome \cite{ji2020action} to curate questions and answers that verify a wide range of reasoning capabilities about human-object interaction, temporal sequence analysis, action prediction, and feasibility inference. Its videos feature single person indoor activities. 
    \item TGIF-QA \cite{jang2017tgif} is an established VideoQA datasets that challenge repeating action recognition, temporal state transition and normal frame QA which invokes a certain frame for answer. The videos are short GIFs and are trimmed to contain only the content of interested for the paired questions. For repeating action and state transition, it provides 5 options for each question and requires the models to pick the correct one. For FrameQA, there is no question-dependent answer options, and the task is to predict each video-question pair with a answer in a globally predefined answer set.
    \item TGIF-QA-R \cite{peng2021progressive} derives from TGIF-QA by fixing the answer bias issue in the tasks of repeating action and state transition. It shares same videos, questions and correct answers with TGIF-QA. In our experiment, we further rectify the redundant issues of the candidate answers in TGIF-QA-R.
    \item MSRVTT-QA \cite{xu2017video} is automatically generated from video descriptions \cite{xu2016msr}. It focuses on a recognition of the video objects and actions (or activities), and each question is answered by one word.
\end{enumerate}
For better understanding of the tasks, we show some typical examples in Fig.~\ref{fig:vis-data}; other statistic details are presented in Tab.~\ref{tab:dset}. For all datasets, we follow standard protocol for experiments and report accuracy (known as percentages of correctly answered questions) as the evaluation metric. 
% Specifically, we report macro-average of accuracy on STAR-QA and micro average of accuracy for other datasets following the original papers.


\subsection{Configuration}
We extract a video at $P\!=\!\{6,15\}$ frames per second for NExT-QA and MSRVTT-QA respectively based on their average video lengths. For TGIF-QA, we extract the GIFs at their default frame rate. For STAR-QA, we follow the original paper and obtain the relevant video segment corresponding to each QA according to the given time stamps; the segments are then treated as independent videos and are extracted at 5 frames per second. We then uniformly sample 8 clips for each video, with a fixed clip length of $z\!=\!16$ frames. Each clip is then further downsampled with a ratio of $\gamma=0.25$. The final clip length is $l=\gamma \cdot z = 4$. For each frame, we detect $n\!=\!10$ regions of high confidence by default (20 for NExT-QA following \cite{xiao2021video}), using the object detection model from~\cite{anderson2018bottom} which was pretrained on the Visual Genome dataset~\cite{krishna2017visual}. The frame appearance feature $F_a$ is extracted from ResNet-101 pretrained on ImageNet. The dimension of the models' hidden states is set to $d=512$, and the default number of graph layers is $U=2$. Besides, the hidden dimension for all transformer blocks is 1024, and the default number of layers and self-attention heads in transformer are $H=1$ and $e=8$ ($e=5$ for edge transformer in DGT) respectively.  


For training with QA annotations, we firstly train the whole model end to end, and then freeze BERT to fine-tune the other parts of the best model obtained at the $1st$ stage. The best results achieved in the two stages are determined as final results. We use hybrid task training for all datasets expect for TGIF-QA which has independent training data for each subtask. We employ Adam optimizer with an initial learning rate $1\times10^{-5}$ and it will degenerate following a cosine annealing schedule with respect to the total iterations. The batch size is set to 64, and the maximum epoch varies from 10 to 30 among different datasets. For pretraining with weakly-paired video-text data, we download about 180K videos (less than 10\%) from WebVid2M
% \footnote{\href{https://m-bain.github.io/webvid-dataset/}{https://m-bain.github.io/webvid-dataset/}}
\cite{bain2021frozen}, and each video is paired with some noisy texts. The videos are then extracted at 5 frames per second and are processed in a same way as for QA. We then optimize the model with an initial learning rate of $5\times10^{-5}$ and batch size 64. The number of negative descriptions of a video for cross-modal matching is set to 63, and they are randomly selected from the descriptions of other videos in the whole training set. Besides, a text token is corrupted at a probability of 15\% in masked language modelling. Following \cite{yang2021just}, a corrupted token will be replaced with 1) the `[MASK]' token by a chance of 80\%, 2) a random token by a chance of 10\%, and 3) the same token by a chance of 10\%. We train the model by maximal 2 epochs which gives to the best generalization results.
% which needs about 2 hours with 4 Tesla V100 GPUs. All code implementation are based on PyTorch.

\subsection{State-of-the-Art Comparison}
In Tab. \ref{tab:resnextqa}, we compare with some strong competitors on NExT-QA.  VGT surpasses the previous SoTA by a clear margin on different tasks, improving the overall accuracy by 2.9\% and 3.7\% on the validation and test sets respectively. Notably, VGT has already shown superior performances even without using external video-text data for pretraining, \eg, it improves the overall accuracy by 1.6\% and 1.9\% respectively. Such strong performance clearly demonstrate the success of our video graph transformer model.

In particular, we analyze the VQA-T method~\cite{yang2021just}, which also solves question answering by ranking instead of classification. VQA-T 
%However, on the one hand, it 
encodes video clips holistically with the S3D representation~\cite{xie2018rethinking} pretrained on HowTo100M \cite{miech2020end}.  % without explicitly modelling the objects and capturing their spatio-temporal interactions. On the other hand, in 
For multi-choice QA, it designs a cross-modal transformer to fuse the video-question pair, but encodes answer candidates independently without the context of the corresponding question. VQA-T achieves good results on descriptive questions that challenge a visual recognition but fails to well answer the causal (\eg~`why' and `how') and temporal (\eg~`before/after') questions. Also, its good performances seriously rely on pre-training with millions of video-text data tailored for QA (\eg~How2VQA69M). When we remove the pre-trained weights learned on How2VQA69M and train the model from scratch, we find that its performances drop sharply on all 3 kinds of tasks as categorised in NExT-QA, especially on tasks challenging dynamic visual reasoning (\eg, causal and temporal questions). 
\setlength{\tabcolsep}{5pt}
\begin{table*}[t]
    \small
    \centering
    \caption{Accuracy (\%) comparison on STAR-QA \cite{wu2021star}.  Acc@I, S, P and F denote accuracy for the tasks of Interaction, Sequence, Prediction and Feasibility respectively. R$^-$: Convolutional feature pretrained on detection tasks. Other results are token from \cite{wu2021star}.}
    \vspace{-0.5em}
    \scalebox{0.9}{
    \begin{tabular}{l|cc|c|c|cccc|c}
    \hline\hline
    \multirow{3}*{Methods} & \multicolumn{2}{c|}{\multirow{1}*{Pretrain}} & \multirow{3}*{Video} & \multirow{3}*{Text} & \multicolumn{5}{c}{STAR-QA Test} \\ \cline{2-3} \cline{6-10}
     ~ & \multirow{2}*{Dataset} & \multirow{2}*{Size} & ~ & ~ & Acc@I & Acc@S & Acc@P & Acc@F & \multirow{2}*{Acc@Mean} \\ 
      ~ & ~ & ~ & ~ & ~ & (35.6\%) & (48.4\%) & (9.1\%) & (6.9\%) & ~ \\ 
    \hline
    NS-SR \cite{wu2021star} & - & - & F, C & GloVe & 30.88 & 31.76 & 30.23 & 29.73 & 30.65 \\ 
    CLEVRER \cite{yi2019clevrer} & - & - &F, C &GloVe & 33.25 & 32.67 & 30.69 & 30.43 & 31.76\\
    \hline
    VisualBERT \cite{li2019visualbert} & - & - & C &BERT & 33.59 & 37.16 & 30.95 & 30.84 & 33.14\\
    LGCN \cite{huang2020location} & - &- &R, F &GloVe & 39.01 & 37.97 & 28.81 & 26.98 & 33.19 \\
    HCRN \cite{le2020hierarchical} & - & - &F, C &GloVe & 39.10 & 38.17 & 28.75 & 27.27 & 33.32 \\
    ClipBERT \cite{fan2019heterogeneous}  &-&  - &R^- & BERT & \underline{39.81} & \underline{43.59} & \underline{32.34} & \underline{31.42} & \underline{36.79} \\ 
    \hline
    \multirow{2}*{\textbf{VGT (Ours)}} & - &- &R, F &BERT & 42.38 & 47.01 & 41.18 & 39.13 & 42.43 \\
    ~ & WebVid & 0.18M &R, F &BERT & {\bf 44.63} & {\bf49.54} & \textbf{43.44} & \textbf{39.65} & {\bf 44.32} \\ \hline
    \multicolumn{5}{c|}{Improvements (\%)} & \textcolor{red}{+4.8} & \textcolor{red}{+6.0} & \textcolor{red}{+11.1} & \textcolor{red}{+8.0} & \textcolor{red}{+7.5} \\ \hline
    \end{tabular}
    }
    \label{tab:resstar}
    \vspace{-0.5em}
\end{table*}

In our model, we introduce video graph transformer which explicitly models the objects and captures their space-time interactions. Our stronger results in both pretraining and pretraining-free settings validates VGT's superiority. Additionally, pretraining VGT demands much less video-text data (\ie, 0.18M \vs 69M) and also dispenses with the need to generate QAs, which is more scalable and adaptable to other tasks like text-video retrieval. Overall, the above analysis concludes that VGT is more data-efficient and more reason-capable video language understanding.

Our model resembles HQGA~\cite{xiao2021video} in constructing local-to-global neural network architecture. A key difference is that HQGA constructs graphs at static frames and does not explicitly model the temporal dynamics, whereas we design dynamic visual graph which explicitly exploits the objects and their relations in adjacent frames to regulate the graphs constructed at static frames. Besides, our graph transformer architecture enables a better compatibility between the visual and textual feature representations, which may potentially benefits cross-modal interaction and matching. Last but not least, HQGA extracts BERT features offline, while we enable online finetuning in an end-to-end fashion. 
We can see from both Tab.~\ref{tab:resnextqa} and Tab.~\ref{tab:resqa} that our method surpasses HQGA on all tasks across different datasets. Such strength of our method comes without the need for pretraining. Furthermore, the stronger results come with more sparse video sampling (\eg, 8 clips each video and 5 regions per frame) and even without using motion feature. The comparison again suggests the absolute superiority of our VGT model to HQGA.

The recent work P3D-G \cite{cherian2022} also designs graph transformer model and has shown great success on NExT-QA (it only reports results on the validation set). However, the transformer is monolithic, and operates over a spatial-temporal graph constructed in a pseudo 3D space. One the one hand, a single monolithic transformer cannot fully reflect the local and global nature of video content. On the other hand, to obtain the pseudo 3D representation of a video and register the objects into it, P3D-G needs to transfer 2D RGB frames into RGB-D ones and merge objects globally throughout a whole video. Both processes will bring additional errors (\eg, accumulate the detection errors) and thus jeopardize the performance. In our model, we design local-to-global graph transformer architectures and only link the object locally within a short video clip.
The results in Tab.~\ref{tab:resnextqa} show that VGT outperforms P3D-G by about 2.9\% and 1.5\% respectively in overall accuracy with and without pretraining. We also notice that P3D-G uses text representations from CLIP \cite{radford2021learning} which is pretrained with large-scale image-text data. As image pretraining helps little in temporal relation reasoning, our method wins remarkably on temporal questions (\eg, from 52.3\% to 56.4\%), demonstrating the strength of VGT in temporal reasoning. 

Tab.~\ref{tab:resstar} shows our results on STAR for visual situated reasoning. We can see that VGT outperforms the previous SoTA (\ie~ClipBERT \cite{lei2021less}) on all the defined four tasks by a clear margin, gaining remarkable improvements of 7.5\% and 5.6\% in mean accuracy with and without pretraining respectively. Again, we find that pretraining steadily boosts performances on all the four tasks defined in STAR, which reveals the strong learning capacity of VGT. We also notice that our results surpasses those neuro-symbolic baselines \cite{wu2021star,yi2019clevrer} which rely on additionally functional programs for supervision. The results demonstrate the superiority of VGT in reasoning about real-world scenes. 

% Finally, we also find that pretraining even hurts VGT's performances on TGIF-QA. We speculate the reasons are two-folds: 1) the task of repeating action identification requires the    

\setlength{\tabcolsep}{8pt}
\begin{table*}[t!]
    \small
    \centering
    \caption{Accuracy (\%) comparison. ViT \cite{dosovitskiy2020image} and VSwin \cite{liu2021video} are recent transformer-style vision encoder. E2E: end-to-end optimized. $\dagger$ denotes our newly curated multiple choices by rectifying the redundant options in TGIF-QA-R\cite{peng2021progressive}. We grey out the results reported in \cite{peng2021progressive} regarding these two tasks as the QAs are slightly different.}
    \scalebox{0.9}{
    \begin{tabular}{l|cc|c|c|ccc|cc|c}
    \hline\hline
    \multirow{2}*{Methods} & \multicolumn{2}{c|}{Pretrain} & \multirow{2}*{Video} & \multirow{2}*{Text} & \multicolumn{3}{c|}{TGIF-QA} & \multicolumn{2}{c|}{TGIF-QA-R} & MSRVTT \\ \cline{2-3} \cline{6-10}
    ~ & Dataset & Size & ~ & ~ & Acton & Trans & FQA & Action^{\dagger} & Trans^{\dagger} & -QA \\ 
    \hline
    STVQA \cite{jang2017tgif} & - & - & F, C & GloVe & 62.9 & 69.4 & 49.5 & - & - & 30.9 \\
    STVQA+ \cite{jang2019video} & -& - & F, C & FastText & 73.5 & 79.7 & 52.0 & - & - & - \\
    CoMem \cite{gao2018motion} & - & - & F, C & GloVe & 68.2 & 74.3 & 51.5 & - & - & - \\
    HME \cite{fan2019heterogeneous} & -& - &F, C &GloVe & 73.9 & 77.8 & 53.8 & \textcolor[rgb]{0.5,0.5,0.5}{\textit{51.9}} & \textcolor[rgb]{0.5,0.5,0.5}{\textit{59.5}} & 33.0 \\
    PSAC \cite{li2019beyond} & - & - & F & GloVe & 70.4 & 76.9 & 55.7 & - & - & - \\
    LGCN \cite{huang2020location}& -&- & R, F & GloVe & 74.3 & 81.1 & 56.3 & - & - & -  \\
    HGA \cite{jiang2020reasoning}& -& - &F, C & GloVe & 75.4 & 81.0 & 55.1 & - & - & 35.5  \\
    QueST \cite{jiang2020divide} & -& - & F, C & GloVe & 75.9 & 81.0 & 59.7 & - & - & 34.6 \\
    HCRN \cite{le2020hierarchical} & -& - &F, C &GloVe & 75.0 & 81.4 & 55.9 & \textcolor[rgb]{0.5,0.5,0.5}{\textit{55.7}} & \textcolor[rgb]{0.5,0.5,0.5}{\textit{63.9}} & 35.6 \\
    HCRN+ \cite{le2021hierarchical} & -& - &F, C &BERT & 69.8 & 79.8 & 57.9 & -& - & 38.3 \\
    B2A \cite{park2021bridge} & - & - & F, C &GloVe &75.9 & 82.6 & 57.5 & - & - & 36.9 \\
    HOSTR \cite{dang2021hierarchical} & -& - & R, F, C &GloVe &75.0 & 83.0 & 58.0 & - & - & 35.9 \\
    HAIR \cite{liu2021hair} & -& - & R &GloVe &77.8 & 82.3 & 60.2 & - & - & 36.9  \\
    MSPAN \cite{guo2021multi} & -& - & F, C & GloVe & 78.4 & 83.3 & 59.7 & - & - & 37.8 \\
    MASN \cite{seo2021attend} & -& - & R, F, C &GloVe & \underline{84.4} & \underline{87.4} & 59.5 &- & - & 35.2 \\
    PGAT \cite{peng2021progressive} & -& - & R, F, C &GloVe &80.6 & 85.7 & 61.1 & \textcolor[rgb]{0.5,0.5,0.5}{\textit{\underline{58.7}}} & \textcolor[rgb]{0.5,0.5,0.5}{\textit{\underline{65.9}}} & 38.1 \\
    HQGA \cite{xiao2021video} & -& - & R, F, C &BERT &76.9 & 85.6 & \underline{61.3} &- & - & \underline{38.6}  \\
    
    \hline
    SSML \cite{amrani2021noise} & HowTo100M & 100M & F, C & W2V & - & - & - & - & - & 35.1  \\
    CoMVT \cite{seo2021look} & HowTo100M & 100M & R, C & BERT & - & - & - & - & - & 39.5 \\
    ClipBERT \cite{lei2021less} & VG+COCO& Human & R$^-$(E2E) & BERT & 82.8 & 87.8 & 60.3 & - & -& 37.4  \\
   
    SiaSRea \cite{yu2021learning} & VG+COCO & Human & R$^-$ (E2E) & BERT & 79.7 & 85.3 & 60.2 & - &- & 41.6 \\
    MERLOT \cite{zellers2021merlot} & YT, CC & 183M & R$^-$, ViT(E2E) & BERT & \underline{94.0} & \underline{96.2} & \underline{\textbf{69.5}} & - & - & 43.1  \\ 
    VIOLET \cite{fu2021violet} &  WebVid & 2.5M & VSwin(E2E) & BERT & 85.5 & 92.1 & - &- & - & - \\
    VIOLET \cite{fu2021violet} &  YT, WebVid, CC & 185M & VSwin(E2E) & BERT & 92.5 & 95.7 & \undeline{68.9} &- & - & {\bf\underline{43.9}} \\ 
    
    \hline
    \multirow{2}*{\textbf{VGT (Ours)}} & - & - &R, F &BERT & {\bf95.0} & {\bf97.6} & 61.6 & 59.9 & 70.5 & 39.7 \\
    ~ & WebVid & 0.18M &R, F &BERT & 93.1 & 97.2 & 61.7 & {\bf60.5} & {\bf71.5} &39.7 \\
    \hline
    \multicolumn{5}{c|}{Improvements (\%)} & \textcolor{red}{+1.0} & \textcolor{red}{+1.4} & \textcolor{red}{-} & \textcolor{red}{+2.0} & \textcolor{red}{+5.6} & \textcolor{red}{-} \\
   
    \hline
    \end{tabular}
    }
    \label{tab:resqa}
\end{table*}
 
In Tab.~\ref{tab:resqa}, we compare our method with previous arts on the TGIF-QA and MSRVTT-QA datasets. The results show that VGT performs pretty well on the tasks of repeating action and state transition in TGIF-QA, surpassing the previous pretraining-free SoTA results significantly by over 10\% (VGT \vs MASN \cite{seo2021attend}: 95.0\% \vs 84.4\% for repeating action identification and 97.6\% \vs 87.4\% for state transition.). It even beats the pretraining SoTA (\ie~MERLOT \cite{zellers2021merlot}) by a non-trivial extent (about 1.0\%), yet without using external data for cross-modal pretraining. By delving into the reason, we find that such strong results are the joint effect of three key designs in our model: the DGT module, the cross-modal interaction mechanism and the strategy of QA by ranking. Please refer to our ablation results in Tab.~\ref{tab:aba} and Fig.~\ref{fig:cm}. Detailed analyses are given in Sec.~\ref{sec:aba}.

Additionally, we conduct an extension experiment on TGIF-QA-R \cite{peng2021progressive} which is curated by making the negative answers in TGIF-QA more challenging. To this end, we firstly fix the `redundant' issue in TGIF-QA-R as we find that there are about 10\% of questions have redundant candidate answers and some of the candidate answers are even identical to the correct one. The results in Tab.~\ref{tab:resqa} show that VGT outperforms the previous SoTA by a clear margin on TGIF-QA-R. The consistently good results on both datasets thus clearly demonstrate the strength of VGT.

Aside from the good performances on the tasks of repeating action and state transition, we find that VGT performs favourably well on the tasks of Frame QA and MSRVTT-QA which challenge a recognition of the visual elements, surpassing previous SoTA in the pretraining-free setting and also showing slightly better results than several models pretrained on millions of video-text data. Nonetheless, we notice that there are still clear gaps between VGT and the SoTA methods (MERLOT \cite{zellers2021merlot} and VIOLET \cite{fu2021violet}). Such inferiority is understandable as we focus on dynamic visual reasoning instead of recognition, and our pretraining data is orders of magnitude smaller than them.

We also observe that pretraining does not help or even slightly hurts the performances on TGIF-QA action and transition tasks. Given that it can effectively improve the results on TGIF-QA-R which shares same GIFs, questions and correct answers. Our reasons are as follows: while pretraining mostly brings good external knowledge, it indispensably involves noises as the data and proxy tasks are not tailored for target tasks. VGT already performs extremely well on target tasks without pretraining, which means that most of the good knowledge from external data can actually be learned from the annotated training data, and thus the involved noises of pretrained model jeopardize the performances. Similar observations are also found in \cite{zoph2020rethinking}, and we refer to it for a detailed discussion of pretraining and self-learning. Indeed, we find the pretraining video-text data (\ie~WebVid) rarely invokes repeating actions and temporal transitions.     

\subsection{Study of Model Components}
\label{sec:aba}
For a better understanding of VGT's success, in this section, we comprehensively study our model designs, including the dynamic graph transformer module, the cross-modal interaction module and some other key implementations that may otherwise sound trivial.

\subsubsection{Dynamic Graph Transformer}
We firstly study the DGT module by substituting it with a simple mean-pooling over the region features; the pooled region features are then interacted with the text features and fed to the global transformer. The ablated model does not capture any spatial and temporal communications between the objects in the local video clips. As shown in the middle part of Tab.~\ref{tab:aba} (w/o DGT), the performances on all datasets drop, especially on these tasks featuring dynamic visual reasoning. For example, the accuracy drops by more than 5\% and 2\% on on TGIF-QA Action and Transition tasks respectively. On NExT-QA and STAR-QA, it drops by 2\% and 3\% respectively. This experiment evinces the vital role of the DGT module.

We then study the effectiveness of temporal graph transformer in DGT by removing both the node and edge transformers defined in Eqn.~\eqref{equ:node} and \eqref{equ:edge}. Thus this ablation considers the graphs that are independently constructed at static frames (depicted in Sec.~\ref{sec:vgr}). The results (w/o GTrans) show that this ablation degenerates the overall accuracy by about 1\% on NExT-QA and 2\% on STAR-QA though it performs better than removing the whole DGT module. Such degeneration mostly comes from a weak performance on answering causal and temporal questions that invoke dynamic visual reasoning. The observations suggest that 1) relations captured at static frames may not be sufficient and accurate though they are effective to boost videoQA performance, and 2) it is important to model the temporal dynamics of the object and their relations. 


We further ablate the graph transformer module to investigate the independent contribution of node transformer and edge transformer. We can see that removing any one of them leads to performance drop (VGT \vs w/o NTrans, VGT \vs w/o ETrans). Also, we find that both transformers help improve the performances separately (w/o GTrans \vs w/o NTrans, w/o GTrans \vs w/o ETrans) in most tasks. By comparing the results of removing the node transformer and edge transformer (w/o NTrans \vs w/o ETrans), we find that the node transformer contributes relatively more to the final results. Such difference is reasonable as 1) the edge of two nodes is depicted by a single value derived from the node representations in our current implementation, and 2) the update of the node representations will also update the edges.

\setlength{\tabcolsep}{4.5pt}
\begin{table*}[t!]
    \small
    \centering
    \caption{Results of model ablation studies.}
    \scalebox{1.0}{
    \begin{tabular}{l|cc|ccc|c|cccc|c}
    \hline\hline
    \multirow{2}*{Model Variants} & \multicolumn{2}{c|}{TGIF-QA}& \multicolumn{4}{c|}{NExT-QA Val} & \multicolumn{5}{c}{STAR-QA Val} \\ \cline{2-12}
    ~ & Action & Trans & Acc@C & Acc@T & Acc@D & Acc@All & Acc@I & Acc@S & Acc@P & Acc@F & Acc@Mean \\ 
    \hline
     VGT & {\bf95.0} & {\bf97.6} & {\bf52.28} & {\bf55.09} & 64.09 & {\bf55.02} & 41.49 & 45.90 & {\bf45.99} & 43.67 & {\bf44.27} \\ \hline
     w/o DGT & 89.6 & 95.4 &  50.10 & 52.85 & 64.48 & 53.22 & 40.58 & 44.92 & 42.15 & 35.94 & 41.15 \\ 
     w/o GTrans & 94.0 & 97.6 & 50.86 & 53.04 & 64.86 & 53.74 & 41.12 & 44.73 & 44.23 & 39.39 & 42.37 \\
     w/o NTrans & 94.5 & 97.4 & 50.79 & 54.22 & 63.32 & 53.84 & 41.45 & 45.65 & 40.87 & 43.47 & 42.86 \\ 
     w/o ETrans & 94.8 & 97.4 & 51.25 & 54.34 & 64.48 & 54.30 & 41.24 & 45.29 & 43.27 & 42.45 & 43.06 \\
     N\&E (Paral) & 93.7 & 97.3 &  51.48 & 54.03 & 64.22 & 54.28 & 41.70 & 44.51 & 44.55 & {\bf44.08} & 43.71 \\
     \hline
     [CLS] & 70.1 & 79.9 & 42.96 & 46.96 & 53.02 & 45.82 & 40.70 &  44.59 & 42.95 & 39.39 & 41.91 \\ 
     w/o F_a & 93.5 & 97.0 & 50.44 & 53.97 & 63.32 & 53.58 & {\bf42.24} & {\bf46.88} & 41.99 & 38.16 & 42.32 \\ 
    
    \hline
    \end{tabular}
    }
    \label{tab:aba}
\end{table*}

\begin{figure*}[t!]
  \begin{center}
    \includegraphics[width=0.95\textwidth]{figures/overfit-crop.pdf}
  \end{center}
  \caption{Investigation of cross-modal interaction.}
  \label{fig:of}
\end{figure*}


Additionally, we study an implementation variant of the graph transformer module by operating the node transformer and edge transformer in parallel on the initial graphs depicted in Sec.~\ref{sec:vgr}. We find that this parallel implementation achieves sub-optimal results compared with our sequential implementation. We speculate that the parallel implementation may jeopardize the graph convolution performance (in Eqn.\eqref{equ:gcn}) since the edges for node communication are not directly derived from the same group of nodes for convolution. 

\subsubsection{Ranking \vs Classification}
We study a model variant by concatenating the outputs of the DGT module (without cross-modal interaction) with the texts' token representations from BERT in a way analogous to ClipBERT \cite{lei2021less}. The formed text-video representation sequence is fed to a cross-modal transformer for information fusion. Then, the output of the ``[CLS]" token is fed to a $|\mathcal{A}|$-way classifier to predict the answer. As can be seen from the bottom part of Tab.~\ref{tab:aba}, this classification model variant ([CLS]) leads to drastic performance drop on all the three datasets. To be complete, we also conduct additional experiments on the FrameQA tasks which is set as open-ended QA. We find that the accuracy of FrameQA drops by nearly 5\% (from 61.6\% to 56.9\%). A detailed analysis of the performances on the training and validation sets (shown in Fig.~\ref{fig:of}) reveals that the model suffer from serious over-fitting on all datasets, especially on NExT-QA and STAR-QA which have relative less number of videos. This experiments demonstrate the superiority of solving QA by relevance comparison between the video-question pair and the candidate answers instead of answer classification.

To further study whether this is caused by the cross-modal transformer or the classification layer. We keep our cross-modal interaction mechanism (introduced in Sec.~\ref{sec:cm}) and discard the cross-modal transformer. Thus, we directly send the cross-modal interacted video representation $f^{vid}$ to a classification layer for multi-choice classification. 
Note that there will be $|\mathcal{A}_{mc}|$ such video representations obtained by interacting the video with different question-answer pairs, and each is mapped to a scalar that gives the probability of the candidate answer to be a correct one. The results in Tab.~\ref{tab:cls} show that this implementation variant (VGT(cls)) wins slightly on the cross-modal transformer (VGT([CLS])). The small improvements could be attributed to that our cross-modal interaction do not involve additional parameters and thus alleviate the over-fitting issue. However, this does not change the fact that a classification setting is sub-optimal for VideoQA.

\setlength{\tabcolsep}{3pt}
\begin{table}[t!]
    \small
    \centering
    \caption{A detailed study of the classification variant.
    }
    \scalebox{1.0}{
    \begin{tabular}{l|ccc|c}
    \hline\hline
    \multirow{2}*{Method} &  \multicolumn{4}{c}{NExT-QA Val} \\ \cline{2-5}
    ~ & Acc@C & Acc@T & Acc@D & Acc@All \\ 
    \hline
    VGT ([CLS]) & 42.96 & 46.96 & 53.02 &  45.82 \\ 
    VGT (cls) &  44.46 & 47.33 & 54.70 & 46.98 \\
    VGT & 52.28 & 55.09 & 64.09 & 55.02 \\ \hline
    \end{tabular}
    }
    \label{tab:cls}
\end{table}

\subsubsection{Cross-modal Interaction}
In Fig.~\ref{fig:cm}, we investigate several implementation variants of the cross-modal interaction module as depicted in Sec.~\ref{sec:cm}. The results suggest that it is better to incorporate textual clues at both the frame- and clip-level outputs (\ie, Eqn.~\eqref{equ:ff} and~\eqref{equ:fc} respectively) for the tasks of repeating action and state transition in TGIF-QA, while a simple interaction at the clip-level outputs (which is our default implementation) brings the optimal results on NExT-QA and STAR-QA. Intriguingly, the region-level interaction seems to be redundant for all experiments. This could be due to that 1) the visual representations at this level are low in semantic space to be compatible with the outputs of BERT, and 2) the frame-level and clip-level representations are actually aggregated from the objects and thus have already absorbed the needed information for interaction. Base on these observations, we plug the cross-modal interaction module at both the frame- and clip-level outputs for TGIF-QA action and transition tasks, and keep the default implementation (interaction at the clip-level) for other datasets, so as to gain both accuracy and efficiency. 
\begin{figure*}[t!]
  \begin{center}
    \includegraphics[width=0.95\textwidth]{figures/inter-crop.pdf}
  \end{center}
  \caption{Investigation of cross-modal interaction.}
  \label{fig:cm}
\end{figure*}

Besides, compared with the baselines that do not use cross-modal interaction, all three kinds of interactions help improve the performances. This is because cross-modal interaction can help identify the relevant visual information from videos for question answering. We notice that the cross-modal interaction improves the accuracies on TGIF-QA by more than 10\%. A possible reason is that the GIFs are trimmed short videos that only contain the visual contents which are relevant to the question-answer pairs. This greatly eases the challenge in spatial-temporal grounding of the positive answer, especially when most of those negative answers are not appear in the short GIFs. Therefore, the cross-modal interaction performs more effectively on this dataset. While the video clips in STAR-QA are also trimmed, its multiple choices are carefully curated to include at least one distractor answer that also appear in the same video clip but is negative to the question. As a result, the improvements are relative smaller.

\subsubsection{Others}
We are interested to know how much the global frame appearance feature helps the performances. The results in the bottom block of Tab.~\ref{tab:aba} (w/o $F_a$) show that $F_a$ contributes steadily to the performances across different datasets. The findings suggest that object-level representation alone may not be sufficient to represent the complex video scene though they are essential to learn object relations. 
In Tab.~\ref{tab:oeqa}, we prove that the QA short-cut in Eqn.~\eqref{equ:oe} can steadily improve the performance. The ablation results show that the accuracy drop on both datasets if we remove the QA short-cut. 
\setlength{\tabcolsep}{3pt}
\begin{table}[t!]
    \small
    \centering
    \caption{Study of the QA short-cut prediction.
    }
    \scalebox{1.0}{
    \begin{tabular}{l|c|c}
    \hline\hline
   Methods & TGIF-FrameQA & MSRVTT-QA \\
    \hline
    VGT & 61.6 & 39.7 \\ 
    VGT w/o QA & 61.2 & 39.1 \\ \hline
    \end{tabular}
    }
    \label{tab:oeqa}
\end{table}

\subsection{Study of Pretraining and Finetuning}
\begin{figure*}[t!]
  \begin{center}
    \includegraphics[width=1.0\textwidth]{figures/pt-crop.pdf}
  \end{center}
  \caption{Pretraining with different size of data. Results are reported on NExT-QA val set.}
  \label{fig:pts}
\end{figure*}

\subsubsection{Number of Pretraining Data}
In Fig.~\ref{fig:pts} we study the QA performances with different size of pretraining data on NExT-QA validation set. Generally, we can see that there is a clear tendency of performance improvements for the overall accuracy (Acc@All) when more data are available. A more detailed analysis shows that these improvements mostly come from a stronger performance in answering causal (Acc@C) and descriptive (Acc@D) questions. It seems that to answer well the descriptive questions, we just need more data for pretraining. However, for answering temporal questions, it demands relative more data to yield positive effect, or otherwise pretraining does not help and even hurts the performance. This could be due to that our pretraining data (\ie~WebVid) rarely invokes temporal descriptions and the proxy tasks are not tailored for temporal reasoning. Finally, answering casual questions is still the most challenging tasks though pretraining helps (The accuracy of causal questions is the lowest among the three tasks as categorised in NExT-QA). Such observations advocate more future efforts in exploring pretraining to better handle temporal and causal reasoning problems, from the aspects of either data or proxy tasks.

\subsubsection{Number of Negative Samples}
\begin{figure}[t!]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{figures/nega-test-crop.pdf}
  \end{center}
  \caption{Contrastive learning with different number of negative samples. Results are reported on NExT-QA test set.}
  \label{fig:ptp}
\end{figure}

In Fig.~\ref{fig:ptp}, we study contrastive learning with different number of negative samples. Our observations are as follows:
\begin{enumerate}
    \item Pretraining the model with different number of negative samples mostly affects the zero-shot QA performances; when finetuning on the target dataset, the differences become smaller (\eg, less than 1\%).
    \item Relatively more negative samples give rise to better results, and the best result is achieved at 63 (by default). Note that the number of negative answers in the target multi-choice QA datasets is 4 or 5, which is much smaller.
\end{enumerate}

\subsubsection{Fine-tuning}
\label{sec:ft}
\setlength{\tabcolsep}{1pt}
\begin{table}[t!]
    \small
    \centering
    \caption{Study of fine-tuning.
    }
    \scalebox{1.0}{
    \begin{tabular}{l|ccc|c}
    \hline\hline
    \multirow{2}*{Method} &  \multicolumn{4}{c}{NExT-QA Val} \\ \cline{2-5}
    ~ & Acc@C & Acc@T & Acc@D & Acc@All \\ 
    \hline
    VGT (QA) &  52.28 & 55.09 & 64.09 & 55.02 \\
    VGT (QA \& MLM) & 49.41 & 54.59 & 64.74 & 53.46 \\ \hline
    VGT (FT QA) &  52.28 & 55.77 & 69.11 & 56.02 \\
    VGT (FT QA \& MLM) &  53.43 & {\bf56.39} & 69.50 & 56.89 \\ \hline
    VGT (FT Adapt All) &  {\bf54.89} & 54.40 & 67.57 & 56.69 \\
    VGT (FT Adapt CD) &  {\bf54.89} & 55.15 & {\bf69.76} & {\bf57.29} \\ \hline
    \end{tabular}
    }
    \label{tab:pt}
\end{table}

\textbf{Masked Language Modelling}. In Tab.~\ref{tab:pt}, we study whether finetuning with masked language modelling (MLM) will also help QA performance. The results show that it can steadily improve the accuracy on all tasks. Nevertheless, when learning the model from scratch on NExT-QA with MLM, such advantage disappears as the results on causal and temporal questions drop though it increases on the descriptive QA task. The observations indicate that it demands more data for learning with masked language modelling on causal and temporal reasoning tasks.

\noindent \textbf{QA Adaptation}. We further study fine-tuning by converting the QA-pairs into descriptions so as to narrow the task gap between pretrain and fine-tune\footnote{We only convert those question whose pattern is clear and easy to adapt, otherwise we directly concatenate the answer behind the question with a separation token `[SEP]'.}, \eg, "why is the baby crying? fell backwards" to "the baby crying [SEP] fell backwards", and "what did the man do after squatting down? wash hands." to "the man [SEP] wash hands [SEP] after squatting down". Our results in Tab.~\ref{tab:pt} (bottom) show that such adaptation benefits the performances on causal questions but hurts others. We speculate the main reason is that the converted descriptions of a particular sample are quite similar for temporal and descriptive questions since their candidate answers are relatively short but they share long question content, which renders it hard to disambiguate between the correct and incorrect answers. Therefore, we have tried another implementation by only adapting the questions that are starting with `why' and `how'. We can see that the overall performance improves. Yet, we find that model does not scale well to the test set (55.08\%). We believe that there are other better adaption methods. As it is not this work's main focus, we leave it for feature exploration.

\subsection{Study of Video Sampling}
In Fig.~\ref{fig:region}, we study the effect of sampled video clips and region proposals on NExT-QA. Regarding the number of sampled video clips, we find that the setting of 8 clips steadily wins on 4 clips, which is understandable as the videos in NExT-QA are relatively long. As for the sampled regions, when learning the model from scratch, the setting of 5 regions gives relatively better result, \eg, 53.68\%. Nonetheless, when pretraining are considered, the setting of 20 regions gives better result, \eg, 55.70\%. Such difference could be due to that learning with more regions can yield over-fitting issues when the dataset is not large enough, since the constructed graph become much larger and more complex. Our speculation is also supported by the fact that the accuracy increases with the number of sampled regions when we only sample 4 video clips and thus less number of graphs.

\begin{figure}[h!]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{figures/invest_clip_region-crop.pdf}
  \end{center}
  \caption{Investigation of sampled video clips and region proposals per frame. Results are reported on NExT-QA test set.}
  \label{fig:region}
\end{figure}

\subsection{Qualitative Analysis}
\begin{figure*}[t!]
  \begin{center}
    \includegraphics[width=0.95\textwidth]{figures/vis-res-t-crop.pdf}
  \end{center}
  \caption{Visualization of prediction results on NExT-QA \cite{xiao2021next}. The ground-truth answers are highlighted in green. }
  \label{fig:vis}
\end{figure*}

\textbf{VGT \vs VGT without DGT}.
As shown in the two examples of Fig.~\ref{fig:vis}(a), the model without DGT is prone to be distracted by the hard negative candidates without the graph transformer module to explicitly modelling the temporal dynamics. For example, to draw a correct answer \texttt{`assemble parts to build toy'}, the model should be aware of a series of boy-toy interactions: \texttt{`tough it'}, \texttt{`grab it'} and \texttt{`plug it into something'}. Although these interactions may happen at different time, they are related to each other and are coordinated to achieve \texttt{`assemble'}. Besides, predictions such as \texttt{`squat down'} require the model to capture the dynamic actions. We can see that the model without dynamic graph transformer tends to predict static thing \texttt{`smiles'} for answer.

\noindent \textbf{VGT \vs VGT with pretraining}.
The examples shown in Fig.~\ref{fig:vis}(b) reveal that pretraining improves the performances on some relatively abstract expressions in the questions and answers, such as \texttt{`help'} and \texttt{'adjust'}. These expressions are natural to human, but their visual correspondences are quite diverse and can hardly learn from limited training data. Yet, such expressions are common in the pretraining data and thus pretraining helps. 

\noindent \textbf{Failure Cases}.
We finally analyze two failure cases in Fig.~\ref{fig:vis}(c). In the first case, we find that the object of interest is too small and the detection model fails to detect it. In the second case, the video is too long and we fail to sample the relevant video clip. In both cases, our model wrongly predict the answers that are semantically close to the questions, \eg, \texttt{`walk down the slope'} \vs \texttt{`stand near the slope'} and \texttt{`stop the black dog'} \vs \texttt{`walk the white dog'}. These observations call for more dense video sampling, but one needs to be careful to balance between the efficiency and accuracy.
